Differentially Private False Discovery Rate Control

Differential privacy provides a rigorous framework for privacy-preserving data analysis. This paper proposes the first differentially private procedure for controlling the false discovery rate (FDR) in multiple hypothesis testing. Inspired by the Benjamini-Hochberg procedure (BHq), our approach is to first repeatedly add noise to the logarithms of the $p$-values to ensure differential privacy and to select an approximately smallest $p$-value serving as a promising candidate at each iteration; the selected $p$-values are further supplied to the BHq and our private procedure releases only the rejected ones. Moreover, we develop a new technique that is based on a backward submartingale for proving FDR control of a broad class of multiple testing procedures, including our private procedure, and both the BHq step-up and step-down procedures. As a novel aspect, the proof works for arbitrary dependence between the true null and false null test statistics, while FDR control is maintained up to a small multiplicative factor.

==> cover.tex <==
Thank you for inviting us to resubmit our paper, Differentially Private False Discovery Rate Control, for publication in the {\em Annals of Statistics}.  We have addressed the helpful criticisms of the referees with great care, and a full description of our responses is contained in a separate attachment.

In the time since our first submission the importance of formal methods for private data analysis, and differential privacy in particular, has only grown.  The US Census Bureau has demonstrated the effectiveness of modern privacy attack methods by applying them to the 2010 published estimates, verifying the results against the confidential data held by the agency.  In response, the bureau has chosen to rely on differential privacy, with its formal proven guarantees, as the confidentiality protection mechanism for the 2020 census.  This, however, is the {\em easy} case, as the decennial form is very short.  The annual Ammerican Community Survey is much, much, more detailed and will need extensive algorithmic work. Privacy loss analysis, independent of differential privacy, has taught us that overly accurate estimates of too many statistics completely destroys privacy -- this is what the bureau exploited in its attack on the 2010 data.  Deciding which estimates to prioritize is a new problem, not only for the census but also for information provided by other statistical agencies.   Differential privacy provides a privacy loss ``budget'' which can be spent safely on selected estimates.   Techniques such as privacy-preserving FDR control will play a significant role in restricting attention - and consumption of the privacy loss budget -- to the estimates that will be of most value.  

The privacy problem is not going away.  At the moment, there is no alternative theory to differential privacy to help with this task.  The questions addressed in this paper will be central to extracting value from data collected at great expense and responder effort.  We believe the results are important and that the messenger matters: publication in the {\em Annals of Statistics} provides unparalleled communication of the message that the field is worthy of the attention of the statistics community.



